Good Data, Large Data, or No Data? Comparing Three Approaches in Developing Research Aspect Classifiers for Biomedical Papers

The rapid growth of scientific publications, particularly during the COVID-19 pandemic, emphasizes the need for tools to help researchers efficiently comprehend the latest advancements. One essential part of understanding scientific literature is research aspect classification, which categorizes sentences in abstracts to Background, Purpose, Method, and Finding. In this study, we investigate the impact of different datasets on model performance for the crowd-annotated CODA-19 research aspect classification task. Specifically, we explore the potential benefits of using the large, automatically curated PubMed 200K RCT dataset and evaluate the effectiveness of large language models (LLMs), such as LLaMA, GPT-3, ChatGPT, and GPT-4. Our results indicate that using the PubMed 200K RCT dataset does not improve performance for the CODA-19 task. We also observe that while GPT-4 performs well, it does not outperform the SciBERT model fine-tuned on the CODA-19 dataset, emphasizing the importance of a dedicated and task-aligned datasets dataset for the target task. Our code is available at https://github.com/Crowd-AI-Lab/CODA-19-exp.

==> sections/discussion.tex <==
%From Tables \ref{tab:4} and \ref{tab:5}, we can see that although we were able to achieve better results than the original PubMed model, it was still not enough to surpass the results obtained using the model trained on CODA-19 dataset. 
%The clear difference between the accuracy using both these models highlights the importance of detailed annotation for such complex tasks. The PubMed data is significantly larger than the CODA-19 dataset, however, for complex tasks, having high-quality annotations may be critical to the success of a machine learning model, even if the dataset is relatively small.

%Using GPT-3, we achieved significantly low results (\Cref{tab:5}) indicating that some presence of well-annotated training data is necessary for this task. As per \cite{gilardi2023chatgpt}, it has been claimed that ChatGPT has been able to outperform crowd-workers for text-annotation. Although this may be an efficient tool for easy tasks (i.e. sentiment classification), our results indicate that for more complicated and detailed tasks such as ours, we need human annotators.

% \paragraph{Querying LLMs.}

